CLIP-TD: CLIP Targeted Distillation for Vision-Language Tasks

Contrastive language-image pretraining (CLIP) links vision and language modalities into a unified embedding space, yielding the tremendous potential for vision-language (VL) tasks. While early concurrent works have begun to study this potential on a subset of tasks, important questions remain: 1) What is the benefit of CLIP on unstudied VL tasks? 2) Does CLIP provide benefit in low-shot or domain-shifted scenarios? 3) Can CLIP improve existing approaches without impacting inference or pretraining complexity? In this work, we seek to answer these questions through two key contributions. First, we introduce an evaluation protocol that includes Visual Commonsense Reasoning (VCR), Visual Entailment (SNLI-VE), and Visual Question Answering (VQA), across a variety of data availability constraints and conditions of domain shift. Second, we propose an approach, named CLIP Targeted Distillation (CLIP-TD), to intelligently distill knowledge from CLIP into existing architectures using a dynamically weighted objective applied to adaptively selected tokens per instance. Experiments demonstrate that our proposed CLIP-TD leads to exceptional gains in the low-shot (up to 51.9%) and domain-shifted (up to 71.3%) conditions of VCR, while simultaneously improving performance under standard fully-supervised conditions (up to 2%), achieving state-of-art performance on VCR compared to other single models that are pretrained with image-text data only. On SNLI-VE, CLIP-TD produces significant gains in low-shot conditions (up to 6.6%) as well as fully supervised (up to 3%). On VQA, CLIP-TD provides improvement in low-shot (up to 9%), and in fully-supervised (up to 1.3%). Finally, CLIP-TD outperforms concurrent works utilizing CLIP for finetuning, as well as baseline naive distillation approaches. Code will be made available.

==> other/backup.tex <==

\begin{itemize}
\item Lots of Vision-Langauge (VL) models have leveraged largely pretraining and delivered impressive performances on popular and competitive VL task leaderboards, e.g. Visual Commonsense Reasoning, Visual Question Answering, Visual Entailment, etc.
\item Since many of those popular VL tasks are highly semantic compared against the traditional single modality task like Visual Recognition, etc, the top-performing models often require fusion modules in order to facilitate the close interaction between modalities during learning.
\item On the other hand, recent work also demonstrated breakthroughs utilizing contrastive loss in largely VL Pretraining. The most famous one, CLIP, was trained on a large amount of visual data guided by language supervision.
\item Their simple dual-independent encoder design allows great flexibility in inputted text format and applying either of its single-modality encoders to downstream tasks. 
\item They prove the generalizability of their transferable visual features by extensive experiments, e.g. they demonstrate results in zero-shot/ few-shot image recognition.
\item However, it is commonly understood that this simple design with independent single-modality encoders may not be suitable for highly multimodal integrated tasks. 
\item These tasks include VCR, VQA, VE, etc., require high integration/interaction between modalities, thus existing methods often require built-in learnable fusion modules to achieve high performance on those tasks. However, CLIP-like models do not have explicit fusion modules but independent encoders for each modality and it hasn’t been proved that this work could clearly deliver promising results on those VL tasks, either. 
\item Based on those, two natural questions come to our attention:
\begin{itemize}
\item Is it feasible to utilize CLIP-like pretraining methods directly to improve on downstream highly multimodal integrated VL tasks?
\item Could we use those CLIP-like pretraining to indirectly help existing V+L fusion models for those VL tasks?
\end{itemize}
\end{itemize}

This work is intended to serve as a wide and comprehensive study to explore the potential of utilizing the popular Vision-Language pretraining with contrastive loss to generalize to downstream general VL tasks, especially the highly semantic visual-question-answering-tasks. Based on our extensive exploration, we also propose a general distillation-based method, Contrastive-Pretraining with Intelligent Knowledge Distillation (CPID). Different from the existing high-performing works, our proposed method could easily be generalized and applied to different existing V-L models without redoing the pretraining step. During our study, we also compare our method against other explored mechanism designs including adapters, ensemble, etc., and existing SOTA methods. Our extensive experiments prove the supremacy of our frameworks that it not only could improve the full-shot performance on downstream tasks but also allow the base models to be more robust and data-efficient in different real-world settings including zero-shot, low-shot, debiased and semi-supervised settings against the SOTA methods.

Our contributions:

\begin{itemize}
    \item First work to extensively explore and analyze zero-shot, low-shot on highly semantic datasets like VCR, VE, and VQA, etc.
    \item We propose a novel and generalized  Intelligent Knowledge Distillation method that could utilize contrastive pretraining to improve on downstream tasks. To the best of our knowledge, our work is the first to propose a method that could generally improve zero-shot/low-shot/full-shot/debiased performance on highly semantic downstream tasks like VCR, VE, and VQA.
    \item We also created innovative methods to create a new debiased evaluation benchmark for Visual Commonsense Reasoning. The new debiased evaluation set based on our methods would be released to the public based on the acceptance of this work.
    \item We conducted extensive experiments to explore and compare the difference among common adaptation mechanisms and SOTA methods. The results show the supremacy of our method and our wide study could also serve as a potential reference for others to apply contrastive pretraining.
    \item Even without redoing large pretraining, our method is able to achieve SOTA comparable results on three different benchmarks

\end{itemize}

